EMinRET: Heuristic for Energy-Aware VM Placement with Fixed Intervals and Non-preemption

Infrastructure-as-a-Service (IaaS) clouds have become more popular enabling users to run applications under virtual machines. This paper investigates the energy-aware virtual machine (VM) allocation problems in IaaS clouds along characteristics: multiple resources, and fixed interval times and non-preemption of virtual machines. Many previous works proposed to use a minimum number of physical machines, however, this is not necessarily a good solution to minimize total energy consumption in the VM placement with multiple resources, fixed interval times and non-preemption. We observed that minimizing total energy consumption of physical machines is equivalent to minimize the sum of total completion time of all physical machines. Based on the observation, we propose EMinRET algorithm. The EMinRET algorithm swaps an allocating VM with a suitable overlapped VM, which is of the same VM type and is allocated on the same physical machine, to minimize total completion time of all physical machines. The EMinRET uses resource utilization during executing time period of a physical machine as the evaluation metric, and will then choose a host that minimizes the metric to allocate a new VM. In addition, this work studies some heuristics for sorting the list of virtual machines (e.g., sorting by the earliest starting time, or the longest duration time first, etc.) to allocate VM. Using the realistic log-trace in the Parallel Workloads Archive, our simulation results show that the EMinRET algorithm could reduce from 25% to 45% energy consumption compared with power-aware best-fit decreasing (PABFD)) and vector bin-packing norm-based greedy algorithms. Moreover, the EMinRET heuristic has also less total energy consumption than our previous heuristics (e.g. MinDFT and EPOBF) in the simulations (using same virtual machines sorting method).

==> fig-algo.tex <==
\begin{algorithm*}[!hbt]
\caption{EMinRET-ST and EMinRET-FT: Heuristics for energy-aware VM allocation in HPC Clouds}\label{alg:remindft}
\begin{algorithmic}[1]

\Function{EMinRET-ST}{}
\State	\textit{Input:} vmList - a list of virtual machines to be scheduled
\State	\textit{Input:} hostList - a list of physical servers
\State	\textit{Output:} mapping (a feasible schedule) or null % \khanh{should be ``null''?. OK}
\State	vmList = sortVmListByStartTime( vmList ) \Comment{1}\label{line:sortbystarttime}
\State return EMinRET( vmList, hostList )
\EndFunction

\Function{EMinRET-FT}{}
\State	\textit{Input:} vmList - a list of virtual machines to be scheduled
\State	\textit{Input:} hostList - a list of physical servers
\State	\textit{Output:} mapping (a feasible schedule) or null % \khanh{should be ``null''?. OK}
\State	vmList = sortVmListByFinishTime( vmList ) \Comment{2}\label{line:sortbyfinishtime}
\State return EMinRET( vmList, hostList )
\EndFunction

\end{algorithmic}
\end{algorithm*}



==> referenc.tex <==
\begin{thebibliography}{4}

%\bibitem{Albers2010} Albers, S. and Fujiwara, H.: Energy-efficient algorithms, ACM Review, Vol. 53, No. 5, pp. 86-96. (2010), doi: 10.1145/1735223.1735245
\bibitem{Albers2010} Albers, S.: Energy-efficient algorithms. Commun. ACM 53(5), 86–96 (2010)

\bibitem{Ittner2007} Barroso, L.A., H\"{o}lzle, U.: The Case for Energy-Proportional Computing. Computer 40(12), 33–37 (2007)

\bibitem{Beloglazov2012} Beloglazov, A., Abawajy, J., Buyya, R.: Energy-aware Resource Allocation Heuristics for Efficient Management of Data Centers for Cloud Computing. Future Generation Computer Systems 28(5), 755–768 (2012)

\bibitem{Beloglazov2011} Beloglazov, A. and Buyya, R.: Optimal Online Deterministic Algorithms and Adaptive Heuristics for Energy and Performance Efficient Dynamic Consolidation of Virtual Machines in Cloud Data Centers, CONCURRENCY AND COMPUTATION: PRACTICE AND EXPERIENCE, Concurrency Computat.: Pract. Exper., pp. 1-24, (2011), doi: 10.1002/cpe

\bibitem{Buyya2009a} Buyya, R., Yeo, C., Venugopal, S., Broberg, J., Brandic, I.: Cloud computing and emerging IT platforms: Vision, hype, and reality for delivering computing as the 5th utility. Future Generation Computer Systems 25(6), 599–616 (2009)

\bibitem{Fan2007a} Fan, X., Weber, W.-D., Barroso, L.A.: Power provisioning for a warehouse-sized computer. ACM SIGARCH Comput. Archit. News. 35, 13 (2007)

%\bibitem{Goiri2010} Goiri, \'{I}., Nou, R., Berral, J., Guitart, J., Torres, J.: Energy-aware Scheduling in Virtualized Datacenters. In: IEEE International Conference on Cluster Computing, CLUSTER 2010, pp. 58–67 (2010)

\bibitem{Hung2011} Quang-Hung, N., Thoai, N., Son, N.T.: Performance constraint and power-aware allocation for user requests in virtual computing lab, Journal of Science and Technology (Vietnam), vol. \textbf{49}, No. 4A, pp. 383-392 (2011.)

%\bibitem{GAPA} Quang-Hung, N., Nien, P. D., Nam, N. H., Tuong, N. H., and Thoai, N..: A Genetic Algorithm for Power-Aware Virtual Machine Allocation in Private Cloud, ICT-EurAsia’13, vol. LNCS \textbf{7804}, pp. 183--191. (2013) doi: 10.1007/978-3-642-36818-9\_19

\bibitem{Hung2013}Quang-Hung, N. et al.: EPOBF: Energy Efficient Allocation of Virtual Machines in High Performance Computing Cloud. J. Sci. Technol. Vietnamese Acad. Sci. Technol. 51, No. 4B, Special on International Conference on Advanced Computing and Applications (ACOMP2013), 173–182 (2013).

\bibitem{HungGPUGA2014} Quang-Hung, N. et al.: A GPU-Based Enhanced Genetic Algorithm for Power-Aware Task Scheduling Problem in HPC Cloud. ICT-EurAsia 2014. LNCS 8407, 159–169 (2014).

\bibitem{Le2011} Le, K. et al.: Reducing electricity cost through virtual machine placement in high performance computing clouds. In: Lathrop, S. et al. (eds.) Proceedings of 2011 International Conference for High Performance Computing, Networking, Storage and Analysis on - SC ’11. p. 1 ACM Press, New York, USA (2011).

\bibitem{Mauch2013} Mauch, V. et al.: High performance cloud computing. Futur. Gener. Comput. Syst. 29, 6, 1408–1416 (2013).

\bibitem{Sotomayor2008} Sotomayor, B., Keahey, K., Foster, I.: Combining batch execution and leasing using virtual machines. In: Proceedings of the Eighteenth International Symposium on High Performance Distributed Computing (HPDC’08), Boston, MA, USA, 23–27 June 2008, pp. 87–96 (2008)

%\bibitem{Sotomayor2009c} Sotomayor, B. and Ignacio, M. and Foster, I.: Resource Leasing and the Art of Suspending Virtual Machines, The 11th IEEE International Conference on High Performance Computing and Communications (HPCC-09),  pp. 59-68. IEEE Computer Society Washington, DC, USA (2009) doi: 10.1109/HPCC.2009.17

\bibitem{Sotomayor2010} Sotomayor, B.: Provisioning Computational Resources Using Virtual Machines and Leases,  PhD Thesis submited to The University of Chicago, US, (2010)

\bibitem{Speitkamp2010} Speitkamp, B., Bichler, M.: A mathematical programming approach for server consolidation problems in virtualized data centers. Serv. Comput. 3, 266–278 (2010)

\bibitem{VonLaszewski2009} von Laszewski, G., Wang, L., Younge, A.J., He, X.: Power-aware scheduling of virtual machines in DVFS-enabled clusters. In: IEEE Intl. Conf. on Cluster Computing and Workshops, 2009, pp. 1–10 (2009), doi:10.1109/CLUSTR.2009.5289182

\bibitem{Panigrahy2011} Panigrahy, R., Talwar, K., Uyeda, L., Wieder, U.: Heuristics for vector bin packing. Technical report, Microsoft Research (2011)

\bibitem{Pham2010} Pham, T.V. et al.: A service composition framework for market-oriented high performance computing cloud. Proceedings of the 19th ACM International Symposium  on High Performance Distributed Computing - HPDC ’10. p. 284 ACM Press, New York, New York, USA (2010).

\bibitem{Feitelson2004} Feitelson, D.G., Rudolph, L., Schwiegelshohn, U.: Parallel job scheduling - a status report. In: Feitelson, D.G., Rudolph, L., Schwiegelshohn, U. (eds.) JSSPP 2004. LNCS, vol. 3277, pp. 1–16. Springer, Heidelberg (2005)

\bibitem{Garg2009} Garg, S.K., Yeo, C.S., Anandasivam, A., Buyya, R.: Energy-Efficient Scheduling of HPC Applications in Cloud Computing Environments. arXiv Prepr. arXiv0909.1146 (2009)

\bibitem{Vis2011} Viswanathan, H. et al.: Energy-Aware Application-Centric VM Allocation for HPC Workloads. 2011 IEEE International Symposium on Parallel and Distributed Processing Workshops and Phd Forum. pp. 890–897 IEEE (2011).

\bibitem{Cloudsim} Calheiros, R.N. et al.: CloudSim: a toolkit for modeling and simulation of cloud computing environments and evaluation of resource provisioning algorithms. Softw. Pract. Exp. 41, 1, 23–50 (2011).

\bibitem{Tako2012} Takouna, I. et al.: Energy efficient scheduling of HPC-jobs on virtualize clusters using host and VM dynamic configuration. ACM SIGOPS Oper. Syst. Rev. 46, 2, 19 (2012).

\bibitem{Maam2011} M\"{a}mmel\"{a}, O. et al.: Energy-aware job scheduler for high-performance computing. Comput. Sci. - Res. Dev. 27, 4, 265–275 (2011).

%\bibitem[Spec1]{Spec1} SPECpower ssj2008 results for Fujitsu Siemens Computers PRIMERGY RX200 S4 (Intel Xeon L5430). \url{http://bit.ly/LvmII4}

%\bibitem{Spec2} SPECpower ssj2008 results for HP ProLiant DL585 G5 (2.70GHz, AMD Opteron 8384). \url{http://bit.ly/JrkskF}

%\bibitem{Spec3} SPECpower ssj2008 results for HP ProLiant DL785 G5 (2.30GHz, AMD Opteron 8376 HE). \url{http://bit.ly/K99RfD}

%\bibitem{SDSC} The San Diego Supercomputer Center (SDSC) Blue Horizon log. \url{http://bit.ly/JUQsiP}
\bibitem{WorkloadLPC} The LPC log from the Parallel Workloads Archive. \url{http://www.cs.huji.ac.il/labs/parallel/workload/l\_lpc/LPC-EGEE-2004-1.2-cln.swf.gz}. Last accessed: 30-January-2014

\bibitem{AmazonEC2HPC}  http://aws.amazon.com/hpc/

\end{thebibliography}

